Dust grains from the heart of supernovae

Dust grains are classically thought to form in the winds of AGB stars. However, nowadays there is increasing evidence for dust formation in SNe. In order to establish the relative importance of these two classes of stellar sources of dust it is important to know what is the fraction of freshly formed dust in SN ejecta that is able to survive the passage of the reverse shock and be injected in the interstellar medium. With this aim, we have developed a new code, GRASH_Rev, that allows to follow the dynamics of dust grains in the shocked SN ejecta and to compute the time evolution of the mass, composition and size distribution of the grains. We consider four well studied SNe in the Milky Way and LMC: SN 1987a, Cas A, the Crab Nebula, and N49. For all the simulated models, we find good agreement with observations. Our study suggests that SN 1987A is too young for the reverse shock to have affected the dust mass. Conversely, in the other three SNe, the reverse shock has already destroyed between 10 and 40% of the initial dust mass. However, the largest dust mass destruction is predicted to occur between 10^3 and 10^5 yr after the explosions. Since the oldest SN in the sample has an estimated age of 4800 yr, current observations can only provide an upper limit to the mass of SN dust that will enrich the interstellar medium, the so-called effective dust yields. We find that only between 1 and 8% of the currently observed mass will survive. This is in good agreement with the values adopted in chemical evolution models which consider the effect of the SN reverse shock. We discuss the astrophysical implications of our results for dust enrichment in local galaxies and at high redshift.

==> tablefootnote/README <==
README for tablefootnote package, 2014/01/08, v1.1a


TABLE OF CONTENTS
=================

1 Introduction
2 Download
3 Installation
4 Additional Packages
5 Package Compatibility
6 Author/Maintainer
7 Bug Reports
8 Known Problems


1 INTRODUCTION
==============

This LaTeX package provides the command \tablefootnote{...}
(and \tablefootnote[...]{...}) to be used in a table
or sidewaystable environment.
In those environments \footnote{...} would not work and
would need to be replaced by \footnotemark in the
(sideways)table and \footnotetext{...} after the
(sideways)table environment ended. Additionally the counters
for footnote and (when the hyperref package with option
hyperfootnotes=true is used) Hfootnote would need to be
adjusted manually. Then still the hyperlinks in a
(sideways)table would not work.
When the footnotebackref package is used, \footnotemark and
\footnotetext{...} would need to be redefined.
Just using \tablefootnote{...} (or \tablefootnote[...]{...})
in the (sideways)table does all this automatically.
(Compatibility with the footnotebackref package was achieved
without redefining \footnotemark or \footnotetext.)
Redefining \footnote was not done as to not create conflicts
with other packages.
This material is subject to the LaTeX Project Public License
(LPPL). See http://www.ctan.org/tex-archive/help/Catalogue/
licenses.lppl.html for the details of that license.


2 DOWNLOAD
==========

`tablefootnote' is available on CTAN:
  CTAN:macros/latex/contrib/tablefootnote/

Running
tex tablefootnote.dtx
generates the files
tablefootnote.ins, tablefootnote.drv, tablefootnote.sty,
and tablefootnote-example.tex.

Also a ZIP file is provided that contains these files,
the manual (tablefootnote.pdf), the compiled example
(tablefootnote-example.pdf), and this README, already
sorted in a TDS tree:
  CTAN:install/macros/latex/contrib/tablefootnote.tds.zip

`CTAN:' means one of the `Comprehensive TeX Archive Network'
nodes or one of its mirrors. This is explained in
  http://www.tex.ac.uk/cgi-bin/texfaq2html?label=archives

The CTAN stuff will be mirrored automatically from the
ftp server, so
  ftp://ftp.tug.org/pub/tex/tablefootnote/
corresponds to
  CTAN:macros/latex/contrib/tablefootnote/


3 INSTALLATION
==============

Installation with ZIP file in TDS format
----------------------------------------
The ZIP file `tablefootnote.tds.zip' contains the files
sorted in a TDS tree. Thus you can directly unpack the
ZIP file inside a TDS tree.
(See CTAN:tds.zip for an explanation of TDS.)
Example:
  cd /...somewhere.../texmf
  unzip /...downloadpath.../tablefootnote.tds.zip
Do not forget to refresh the file name database of this
TDS tree.
Example:
  texhash /...somewhere.../texmf

Manual installation
-------------------
a) Download the tablefootnote files from CTAN.
   If necessary, unpack them.
b) Generate the package and driver files:
     tex tablefootnote.dtx
c) Install the file `*.sty' in your TDS tree:
     cp *.sty TDS:tex/latex/tablefootnote/
   Replace `TDS:' by the prefix of your TDS tree
   (texmf directory).
d) Create the documentation (if necessary), e.g.
     pdflatex  tablefootnote.dtx
     makeindex -s gind.ist  tablefootnote.idx
     pdflatex  tablefootnote.dtx
     makeindex -s gind.ist  tablefootnote.idx
     pdflatex  tablefootnote.dtx
e) Update the databases if necessary, e.g. for teTeX:
     mktexlsr .../texmf
f) Create the tablefootnote-example.pdf (if necessary), e.g.
     pdflatex tablefootnote-example.tex
     pdflatex tablefootnote-example.tex
     pdflatex tablefootnote-example.tex
g) Copy the documentation files to
   "TDS:doc/latex/tablefootnote/":
   README, tablefootnote.pdf, tablefootnote-example.tex,
   tablefootnote-example.pdf.


4 ADDITIONAL PACKAGES
=====================

tablefootnote loads other packages:
* letltxmacro, http://ctan.org/pkg/letltxmacro
* ltxcmds, http://ctan.org/pkg/ltxcmds
* xifthen, http://ctan.org/pkg/xifthen
When the etoolbox package is available, it is used:
* etoolbox, http://ctan.org/pkg/etoolbox
(All packages possibly load further packages.
See the result of the \listfiles command in the log-file
of the example.)


5 PACKAGE COMPATIBILITY
=======================

- Using the hyperref-option pdfview=FitH or FitBH makes the
    hyperlinks of footnotes in sidewaystables to not lead
    to the footnotes, due to a bug in pdfTeX,
    computing wrong anchor coordinates (Heiko Oberdiek,
    29. October 2011). The printed version is OK.
- Footnotes in sidewaystables are printed one below the
    other, even if the footmisc package with option "para"
    is used.
- When LuaTeX is used to compile a document with
    rotated content, the hyperreferences therein are
    misplaced (regardless of loaded tablefootnote-package
    or footnotes at all - all hyperreferences in
    rotated content are misplaced). Using pdflatex does not
    result in any problem here.


6 AUTHOR/MAINTAINER
=====================

* H.-Martin Münch


7 BUG REPORTS
==============

A bug report should contain:
* Comprehensive problem description. This includes error or
  warning messages.
* \errorcontextlines=\maxdimen can be added in the
  TeX code to get more information in TeX error messages.
* Minimal test file that shows the problem, but does not
  contain any unnecessary packages and code.
* Used drivers/programs.
* Version information about used packages and programs.
* If you are using LaTeX, then add "\listfiles". Then
  a list of version information is printed at the end
  of the LaTeX run.
* Please no other files than the minimal test file.
  The other files .log, .dvi, .ps, .pdf are seldom
  necessary, so send them only on request.
* Please .zip or .tar.gz your file(s) before sending them!

Bug address
-----------
Bug reports can be send to the maintainer:
  H.-Martin Münch
  <Martin [dot] Muench [at] Uni-Bonn [dot] de>


8 KNOWN PROBLEMS
=================

- Using the hyperref-option pdfview=FitH or FitBH makes the
    hyperlinks of footnotes in sidewaystables to not lead
    to the footnotes, due to a bug in pdfTeX,
    computing wrong anchor coordinates (Heiko Oberdiek,
    29. October 2011) The printed version is OK.
- Footnotes in sidewaystables are printed one below the other,
    even if the footmisc package with option para is used.
- When a table with (table)footnotes floates to another place,
    its footnotenumbers are not automatically adapted.
- When LuaTeX is used to compile a document with
    rotated content, the hyperreferences therein are
    misplaced (regardless of loaded tablefootnote-package
    or footnotes at all - all hyperreferences in
    rotated content are misplaced). Using pdflatex does not
    result in any problem here.

Ideas for solutions are welcome!
